Randomized Broadcast in Radio Networks with Collision Detection

We present a randomized distributed algorithm that in radio networks with collision detection broadcasts a single message in $O(D + \log^6 n)$ rounds, with high probability. This time complexity is most interesting because of its optimal additive dependence on the network diameter $D$. It improves over the currently best known $O(D\log\frac{n}{D}\,+\,\log^2 n)$ algorithms, due to Czumaj and Rytter [FOCS 2003], and Kowalski and Pelc [PODC 2003]. These algorithms where designed for the model without collision detection and are optimal in that model. However, as explicitly stated by Peleg in his 2007 survey on broadcast in radio networks, it had remained an open question whether the bound can be improved with collision detection. We also study distributed algorithms for broadcasting $k$ messages from a single source to all nodes. This problem is a natural and important generalization of the single-message broadcast problem, but is in fact considerably more challenging and less understood. We show the following results: If the network topology is known to all nodes, then a $k$-message broadcast can be performed in $O(D + k\log n + \log^2 n)$ rounds, with high probability. If the topology is not known, but collision detection is available, then a $k$-message broadcast can be performed in $O(D + k\log n + \log^6 n)$ rounds, with high probability. The first bound is optimal and the second is optimal modulo the additive $O(\log^6 n)$ term.

==> MultiMessage-NC.tex <==
\section{Multi-Message Broadcast in Known Topology Setting}\label{sec:multiBC}
In this section, we present a multi-message broadcast algorithm that, given a GST, broadcasts $k$ messages in $O(D +k \log n + \log^2 n)$ rounds. To the best of our knowledge, this is the first algorithm to achieve achieves this asymptotically optimal running time (even) in the known topology scenario. 

%This section is organized as follows. In \Cref{sec:schedule} we modify the gathering BFS-tree schedule from \cite{GPX} to allow the streamlined broadcast of not just one but multiple messages. In \Cref{sec:NCalgorithm}, we combine this schedule with the standard distributed implementation of random linear network coding (RLNC). While the algorithm is relatively easy to describe its analysis requires the use of recent advances in analyzing network coding performance from \cite{Haeupler11} in a novel way, which we call \emph{backwards projection analysis}. We describe network coding in \Cref{sec:NCintro} and explain the backwards projection analysis on a simpler example in \Cref{sec:NCanalysis} before we give the complete analysis of our network coding algorithm in \Cref{sec:NCalgorithm}. % and discuss the possibility of replacing the network codes in our fast implementation by forward error correction codes, a simpler form of coding.

%We also show that using only forward error correction codes at the source and sinks it is possible to almost match the performance of network coding with a $O(D +k \log n + \log^2 n) \log \log n$ and give a candidate that might remove the additional $\log \log n$ factor.

\subsection{Ranom Linear Network Coding and Backwards Projection Analysis}
In this subsection, we recap on the definition of random linear network coding and present a simple network coding algorithm to broadcast $k$ messages in $O((D + k \log n + \log n)\log n)$ rounds, with high probability. This simple algorithm provides a good substrate for us to present the backwards projection analysis in a simpler setting.

We later explain that this algorithm can be improved to $O(D + k \log n + \log^2 n)$ using a combination of network coding and the GST trees, using a novel transmission schedule on GST trees tailored for multi-message case.


\subsubsection{Random Linear Network Coding}\label{sec:NCintro}

Using network coding, nodes can mix messages before forwarding. This is in contrast with the traditional ``store and forward'' paradigm in which messages are simply forwarded without being combined. One of the benefits of using network coding is in increasing capacity in networks.

Network Coding was introduced by Ahlswede et at. \cite{ACLY} and extended to RLNC by \cite{HKMKE}. There also a distributed implementation for network coding was suggested. The first use of network coding in gossip-type information dissemination was in \cite{deb2006algebraic}. Lastly, the projection analysis used here can be found in \cite{Haeupler11}.

%\iffalse
%When routing, a node that has multiple messages and is sending has to decide which message to send. This can become a bottleneck, since in a broadcast setting each of its receivers might need a different message.
%%The idea of RLNC network is to send a (random linear) mixture of all messages a node has.
%For example, consider the setting setting where a node $v$ is connected to $k$ other nodes and knows all $k$ messages, while each of its neighbors knows a different subset of $k-1$ out of the $k$ messages. When routing messages, it takes at least $k$ transmissions of $v$ to inform all its neighbors about the missing message. A more efficient solution is to send the XOR of all $k$ messages. Upon receiving this in the first round, each neighbor can XOR the $k-1$ messages it has, and thus obtain the one missing message it needs.
%Linear network coding generalizes this idea to networks.
%\fi

In random linear network coding, a message is regarded as a vector $\vec{m}$ over a finite field $\Fq^l$, where $q$ is an arbitrary prime or prime power.
In the setting of multiple messages $\vec {m_1},\ldots,\vec {m_k}$ network coded packets consist of a linear combination of messages $\vec m = \sum_{i=1}^k \mu_i \vec {m_i} \in \Fq^l$ and a vector of coefficients $\vec \mu = (\mu_1,\ldots,\mu_k) \in \Fq^k$. Because of linearity, a node that knows some of these packets can create a packet of this form for any coefficient combination that is spanned by the coefficient vectors of the packets (and messages) known to it. Also, given a set of $k$ packets with linearly independent coefficient vectors one can reconstruct all messages using Gaussian elimination. Now, the algorithm can be simply described:

Every node $u$ stores all received packets, and maintains the subspace that is spanned by them. Whenever a node decides to transmit, it chooses a random coefficient vector from the subspace by taking a random linear combination of the coefficient vectors stored, and creates a new packet to transmit. Every time a node receives a new packet, it updates its subspace, and if the subspace spanned by the coefficient vectors is the full space, it reconstructs all messages.

%\iffalse
%\bcomment{This is a paste and copy from an earlier NC paper so some reformulation is needed}
%
%The RLNC algorithm sends out packets in the form of vectors over a finite field $\Fq$, where $q$ is an arbitrary prime or prime power. We assume that there are $k$ messages, $\vec {m_1},\ldots,\vec {m_k}$, that are vectors from $\Fq^l$ of length $l$. Every packet that is sent around during the execution of the algorithm has the form $(\vec \mu,\vec m)$, where $\vec m = \sum_{i=1}^k \mu_i \vec {m_i} \in \Fq^l$ is a linear combination of the messages, and $\vec \mu = (\mu_1,\ldots,\mu_k) \in \Fq^k$ is the vector of the coefficients. If enough packets of this form are known to a node, i.e., the span of the coefficient vectors is the full space $\Fq^k$, Gaussian elimination can be used to reconstruct all messages. For this, only $k$ packets with linearly independent coefficient vectors are needed. Linearity furthermore guarantees that any new packet that is created by taking a linear combination of old packets has the same valid format. With this, it is easy to see that a node can produce any packet whose coefficient vector is spanned by the coefficient vectors of the packets it knows. The algorithm is now easily described:
%
%Each node $v$ maintains a subspace $X_v$ that is the span of all packets known to it at the beginning and received so far by simply storing all received packets. If $v$ does not know any messages at the beginning, then $X_v$ is initialized to contain only the zero vector. If $v$ knows some message(s) $\vec m_i$ at the beginning, $X_v$ is initialized to contain the packet $(\vec \mu,\vec {m_i})$ in which $\vec \mu$ is the $i^{\text{th}}$ standard basis vector. $X_v$ also contains all linear combinations that complete the span of these packet(s).
%Whenever node $v$ sends out a packet, it chooses a uniformly random packet from $X_v$ by taking a random linear combination of the stored packets. At the end of each round, all received packets are added to $X_v$ and again the span is taken. If the subspace spanned by the coefficient vectors is the full space, a node decodes all messages.
%
%\bcomment{End of copy}
%\fi


\subsubsection{Backwards Projection Analysis}\label{sec:NCanalysis}

In this section, we show that, network coding can be used with a simple BFS-tree schedule to disseminate $k$ messages in $O((D + k + \log n) \log n)$ rounds. This is interesting in its own right and also serves as a simple way to explain our new backwards projection analysis in isolation. This is a helpful preparation for the next part where we will use this analysis together with the more complicated MGBFS-schedule to obtain the optimal $O(D)$ dependence. 

Here, we assume the single-source broadcast setting in which all $k$ messages are initially at the source node $s$.
We furthermore assume that each node $u$ knows its distance $l_u$ to $s$. Having this, nodes communicate in phases.
A phase starts with all nodes at level $l \equiv 0 \pmod{3}$ performing a $\log n$ round iteration of the Decay algorithm,
that is, broadcasting with probability $2^{-i}$ with $i$ varying from $1$ to $\ceil{\log_2 n}$.
To complete a phase, the same process is repeated for all nodes $u$ with distance $l_u \equiv 1 \pmod{3}$, and then for all nodes $u$ with distance $l_u \equiv 2 \pmod{3}$. Whenever a node decides to send, it uses the network coding protocol described in \Cref{sec:NCintro} to construct the packet.

\begin{lemma}\label{lem:simpleNC}
Broadcasting $k$ messages from $s$ to all nodes takes, with high probability, $O((D + k + \log n) \log n)$ rounds, where $D$ diameter of the network.
\end{lemma}

We will use the projection technique from \cite{Haeupler11} to analyze the propagation of knowledge during the random linear coding procedure. In essence this technique only requires to show that one message floods the network sufficiently fast if every node knowing it sends out packets that are informative about the message, with constant probability. An exponential tail bound on this flooding process then directly gives results for $k$ messages. Note that this is exactly the flooding process analyzed \cite[Claim 3.2.]{GPX05} and many other places \underline{except} that we now have to assume that nodes that are scheduled to send but do not know the message are sending noise are thus still causing collisions. This makes a big difference and kills the original analysis. While it is a priori not clear that information still spreads quickly we recover something closely resembling the original proof using our new backwards analysis. 
 
{
For the projection analysis part of the proof we need the following crucial definition and easy to verify facts:

\begin{definition}[{\cite[Definition 4.1.]{Haeupler11}}]
A node knows a coefficient vector $\mu \in GF(2)^k$ if it has received a packet with a coefficient vector $c \in GF(2)^k$ that is not orthogonal, that is, $\left\langle \mu,c \right\rangle \neq 0$.
\end{definition}


\begin{proposition}[{\cite[Lemma 4.2.]{Haeupler11}}]\label{prop:NCfacts}
If a node knows a coefficient vector and sends a packet to a node $v$ then this node $v$ afterwards knows $\mu$ with probability at least $1/2$. Furthermore, if a node knows all $2^k$ coefficient vectors it can decode.
\end{proposition}

\begin{proof}[Proof of \Cref{lem:simpleNC}]
We claim that for any non-zero vector $\mu$ the probability that any fixed node $v$ does not learn $\mu$ within $O((D + k + \log n)\log n)$ rounds is at most $2^{-(k + 2 \log n)}$. From this we conclude via a union bound over all $2^k$ coefficient vectors and all nodes that with high probability all nodes know all coefficient vectors. It then follows from \Cref{prop:NCfacts} that all nodes can decode.

For a node $v$ to learn a fixed coefficient vector $\mu$ there has to exist a sequence of collision-free transmissions from $s$ to $v$. Furthermore, these transmission must carry a coefficient vector that is non-orthogonal to $\mu$. According to \Cref{prop:NCfacts} for any given collision-free transmission there is an independent $1/2$ probability for this to happen. These probabilities are not just independent between each other but are also independent from which nodes send and receive (collision-free) transmissions. We can thus assume that first all collision-free transmissions are determined and then independently each such transmission fails (with respect to $\mu$) with probability $1/2$. Given this we show next that one can find a succesful sequence of transmissions from $s$ to $v$ with probability at least $1 - 2^{-(k + 2 \log n)}$. We will analyze the progress of finding such a sequence by going backwards in time. While this seems not to make a big difference it is crucial and makes the proof that would otherwise seem doomed almost magically easy.

More precisely, our backwards analysis looks at times between $T$ and $1$ and defines a node $v$ at level $l$ to have $d$ successes at time $t$ if there is a node $u$ at level $l-d$ such that there is a sequence of successful and collision-free transmission from $u$ to $v$ between time $t$ and $T$. Thus at most $D$ successes are needed for a node $v$ to learn $\mu$. Furthermore, we will show that in each phase any node $v$ has a constant probability to land at least one success. For this let $v$ have $d$ successes so far and let $u$ be a node with on level $l-d$ having the sequence of successful and collision-free transmission to $v$. Between $t - 3\ceil{\log_2 n}$ and $t$ there is a full iteration of the Decay protocol performed by the nodes in level $l-d-1$ and according to \Cref{lem:progfast} there is thus a constant probability that $u$ receives a collision-free transmission from one of these nodes. With constant probability this transmission is furthermore successful with respect to $\mu$. Therefore there is always an independent constant probability for each phase to generate a success. After $\Theta(D + k + \log n)$ phases the expected number of successes is thus $\Theta(D + k + \log n)$ and due to standard Chernoff bounds the chance that there are less than $D$ successes is at most $2^{-\Theta(D + k + \log n)}$.
\end{proof}

}

\subsection{The Modified Transmission Schedule for GSTs}\label{sec:schedule}

Our framework is essentially taking the transmission schedule of \cite{GPX05} used on top of GST and extending it to multiple messages. This idea was also attempted in \cite{GP} but its correctness was disproved \cite{QinPersonalCommunication}.

Unfortunately while the schedule in \cite{GPX05, GP} works well in transmitting one message, it cannot be used to pipeline multiple messages directly. The reason is that the analysis of \cite{GPX05} which proves progress of propagation along the tree relies crucially on the fact that nodes that are supposed to send but do not know the message remain silent. This is not possible when multiple messages are to be transmitted since these nodes are making progress on other messages. Instead we modify the schedule of \cite{GPX05} to continue making progress on one message even if other senders (which do not know the message) send noise instead of being silent. In the following, we explain our transmission schedule for broadcasting multiple messages atop GST.

%We use a gathering rank-labeled BFS-tree as introduced in \cite{GPX05}. A rank-labeled BFS-tree is a BFS-tree rooted at the source $s$. We assume the standard notions of levels and parent-child-descendant relationships. We assign each node a rank by the following inductive labeling rule: Each leave has rank $1$; a node with $l$ children of rank $r_1 \geq r_2 \geq \ldots \geq r_l$ has a rank $r_1$ if $r_1 > r_2$ and $r_1+1$ otherwise. A rank-labeled BFS-tree is called gathering if any node of rank $i$ on level $l$ is adjacent to at most one node of rank $i$ at level $l-1$. The existence of such a gathering rank-labeled BFS-tree was proven in \cite{GPX05}:
%
%\begin{lemma}[\cite{GPX05}]\label{lem:gathering}
%For any graph and any node $s$ a gathering rank-labeled BFS-tree rooted at $s$ can be found in polynomial time. Furthermore, the maximum rank of any rank-labeled BFS-tree is at most $\ceil{\log_2 n}$.
%\end{lemma}

The labeling of the gathering BFS-tree defines stretches along which messages can get pipelined fast. In particular, it is possible to pipeline messages along tree-paths that have the same rank without conflicts. We add special directed edges indicating these fast transmission paths. More formally, for a graph $G$ and a gathering spanning tree $T$, we create an imaginary graph $G'$ as follows: we add a directed fast edge from every node $u$ with rank $r$ at level $l$ to every descendant of $u$ in $T$ with rank $r$. We note that, while the diameter of $G$ is $D$, the shortest (directed) path from $s$ to every node $u$ in $G'$ is at most $2\ceil{\log_2 n}$ long. To see this, consider the path from $u$ to $s$ in $T$. On this path, the rank never decreases, thus increases at most $\ceil{\log_2 n}$ times. Furthermore, every stretch on which the rank stays the same corresponds to a directed link in $G'$. Using this, we get the path of length at most $2\ceil{\log_2 n}$ from $s$ to $u$ in $G'$. We use the notation $d_u$ to denote the length of the shortest (directed) path from $s$ to $u$ in $G'$. Thus, $d_u \leq 2\ceil{\log_2 n}$. Equipped with these three labels -- $l_u$ (the BFS layers), $r_u$ (the ranks in the GST) and $d_u$ (the directed distance from the source $s$ in $G'$), we can now define the following schedule \emph{modified gathering BFS-tree (MGBFS) schedule}:

%create a collision free schedule using a modification of the method in \cite{GPX05}.

\begin{definition}[MGBFS schedule]\label{def:schedule}
Given a graph $G$ with a rank-labeled gathering BFS-tree $T$ and a distance label $d$ of $G'$, the MGBFS schedule is defined as follows:
%At the beginning of each round $t$ and each level $l$ we draw a uniformly random integer $i_{t,l}$ from $\{1,2,\ldots,\ceil{\log_2 n}\}$.
The schedule alternates between fast and slow transmissions with fast transmissions only happening when $t \equiv 0 \pmod{2}$ and slow transmissions only happening when $t \equiv 1 \pmod{2}$.
A node $u$ at level $l$ with rank $r$ and distance label $d$ performs a fast transmission if $t \equiv 2(l + 3r) \pmod{6\ceil{\log_2 n}}$, and a slow transmission with probability $2^{-((t-1-2d)/6 \mod \ceil{\log_2 n})}$
if $t \equiv 1 + 2d \pmod{6})$.
\end{definition}

We note that the MGBFS schedule uses fast exchanges exactly as before to pipeline messages towards nodes far away from the source in $G$. The main and crucial modification of the schedule compared to \cite{GPX05,GP} lies in defining the levels of slow exchanges with regards to $G'$ and not $G$. This results in slow exchanges not trying to push messages away from the source themselves but instead they tend to push messages towards entry points of fast stretches (even if this results in going backwards). While this modification on the schedule is only minor a new potential based backwards analysis is needed to prove that this schedule remains efficient even if uninformed nodes broadcast noise.

To prove the new schedule efficient we first show that it is collision free:

\begin{lemma}
In MGBFS schedule, there are no collisions between any two fast transmissions or between any fast and any slow transmission.
\end{lemma}
{
\begin{proof}
Since fast and slow transmission only happen during even and odd rounds, respectively, it is clear that collisions can only happen between two slow or two fast transmissions.
To see that two fast transmission do not collide, we note that only levels $l$ with $l \equiv t/2 \pmod{3}$ have transmissions since for a fast transmission to happen we need at least $t \equiv 2l + 6r \equiv 2l \pmod{6}$. Since nodes whose levels differ by at least $3$ can not share a neighbor this guarantees that collisions are only caused by nodes within the same level. Two nodes within the same level are furthermore only performing a fast transmission if their ranks $r$ and $r'$ are equivalent modulo $\ceil{\log_2 n}$. By definition of GST, this implies that their ranks are equal and the \emph{collision-freeness} property of GST then guarantees that two such nodes do not share a neighbor in the next level. This shows that there are indeed no collisions between any two fast transmission.
\end{proof}
}

In the absence of collisions for fast transmission one can see from \Cref{def:schedule} that fast transmissions pipeline nicely. We will use this pipelining to quickly transmit messages from the node at the beginning, that is with smallest level $l$, of a fast-stretch to all nodes on the stretch. For this we make the following rule. Whenever a node in the middle of a fast stretch has to send a message it chooses to relay the last message it has received during a fast transmission from its parent in $T$. This way we get the following property:

\begin{lemma}\label{lem:progslow}
In MGBFS schedule, if node $u$ with level $l$ is the beginning of a fast stretch in $T$ sends a message at time $t$ during a fast transmission then any node $v$ with level $l'>l$ on the same fast stretch will receive this message not later than at time $t' = t + 2(l'-l)$.
\end{lemma}

\noindent
For slow transmissions we get the following progress guarantee:

\begin{lemma}\label{lem:progfast}
For any node $u$ with distance label $d$ if there is at least one node $v$ connected to $u$ in $G$ with distance label $d-1$ then with probability at least $\frac{1}{2e}$ node $u$ receives a message from one such node within any fixed span of $6\ceil{\log_2 n}$ rounds.
\end{lemma}
{
\begin{proof}
Let $x$ be the number of neighbors of $u$ with distance label $d-1$. Note that within any span of $6 \ceil{\log_2 n}$ rounds there is a round in which all nodes in level $d-1$ send a message independently with probability $p$ between $\frac{1}{x}$ and $\frac{1}{2x}$ while all nodes with distance label $d$ and $d+1$ and thus also all other neighbors of $u$ are silent. The probability that $u$ receives a message from any particular neighbor in this round is at least $\frac{1}{2x} (1 - \frac{1}{x})^{x-1} > \frac{1}{2ex}$. These events are mutually exclusive and we thus get that the total probability for at least one neighbor successfully transmitting to $u$ during this round is at least $\frac{1}{2e}$.
\end{proof}
}



\subsubsection{Optimal Network Coding Broadcast}\label{sec:NCalgorithm}

In this section, we show that using the network coding protocol of \Cref{sec:NCintro} to create packets for the MGBFS schedule results in a fast broadcast algorithm.

The algorithm description is simple.
We use the MGBFS to decide which node sends at what round.
Each time a node decides to sent, it creates a packet using network coding by combining the messages it has received earlier.
Note that we still stick with the rule that intermediate nodes in a fast stretch do {\em not} create packets for a fast transmission, but simply relay the message they received during the fast transmission round.

\begin{lemma}
Suppose we use the MGBFS schedule with random linear network coding to transmit $k$ messages from the source $s$ to all nodes. Then, with high probability, after $O(D + k\log n + \log^2 n)$ rounds all nodes can decode all messages.
\end{lemma}

{
\begin{proof}
As in the proof of \Cref{lem:simpleNC}, we will use the projection technique of \cite{Haeupler11} and analyze the spreading of one coefficient vectors $\mu$ to one node $v$. We do this again by going backwards in time and finding a path of collision-free transmission from $v$ to the source $s$ that is successful \emph{with respect to} $\mu$.
We show that $T = O(D + k\log n + \log^2 n)$ rounds suffice to find such a path with probability at least $1 - 2^{-(2\log n + k)}$.
As before, a union bound over all nodes and all vectors then finishes the proof, and shows (together with \Cref{prop:NCfacts}) that every node can decode.

For any $t$, going backwards in time from time $T$, we will track the set $U_t$ of nodes that are connected to $v$ by a sequence of successful and collision-free transmissions. We then define the potential of $v$ at time $t$ to be $\min_{u \in U_t} d_u \ceil{\log_2 n} + l_u$. We will show that this potential decreases with probability at least $\frac{1}{4e}$ by at least $\ceil{\log_2 n}-1$ every $8\ceil{\log_2 n}$ rounds.

We start with the case where the node $u \in U_t$ that minimizes the potential of $v$ has at least one neighbor at level below it in $G'$. In this case, \Cref{lem:progslow} guarantees that with probability at least $\frac{1}{2e}$ during the rounds between $t - 6 \ceil{\log_2 n}$ and $t$ there is a collision-free transmission from a node $u'$ with $d_{u'} = d_u - 1$ to $u$, and is successful with respect to $\mu$, with probability $1/2$.
Since $u'$ and $u$ are neighbors their levels $l_u$ and $l_{u'}$ differ at most by one, thus a successful transmission decreases the potential by at least $(d_u \ceil{\log_2 n} + l_u) - (d_{u'} \ceil{\log_2 n} + l_{u'}) = (d_u - d_{u'})\ceil{\log_2 n} - (l_u - l_{u'}) \geq \ceil{\log_2 n} - 1$. Thus, if $u$ has a neighbor with a distance label lower than $d_u$
then with probability at least $\frac{1}{4e}$ the potential decreases by at least $\ceil{\log_2 n} - 1$ within any $8 \ceil{\log_2 n}$ rounds.

In the second case, the node $u \in U_t$ that minimizes the potential of $v$ at time $t$ does not have a neighbor with a lower distance label.
For this case, we need to understand the behavior of fast stretches. We first observe that the start node of any fast stretch initiates a ``transmission wave'' every $6 \ceil{\log_2 n}$ rounds by creating a new message and sending it as a fast transmission. This message gets then pipelined through the fast stretch with one progress every fast transmission rounds (that is every two rounds) until the message reaches the end of the stretch. For any node on a fast stretch there is thus a new wave arriving every $6\ceil{\log_2 n}$ rounds and each of these waves is successful with respect to $\mu$ with probability at least $1/2$.

Note that the second case can only happen if $u=s$ or if there is one directed edge in $G'$ representing a fast stretch going into $u$ originating from a node $u'$ one level below $u$ in $G'$.
Thus, at a time $t'$ between $t-6 \ceil{\log_2 n}$ and $t$, a fast transmission wave arrives in $u$ and with probability $1/2$ leads to an extended sequence of collision-free transmissions that are successful $\mu$.
In particular, if the wave originated from $u'$ during the rounds $t'-2 \ceil{\log_2 n}$ and $t'$ then there is a sequence of transmission from $u'$ to $v$ between time $t - 8 \ceil{\log_2 n}$ and $T$, and otherwise the wave propagated for $\ceil{\log_2 n}$ steps and there is a node $u''$ between $u'$ and $u$ on the fast stretch with a sequence of transmission to $v$ starting at time $t - 8 \ceil{\log_2 n}$. In both cases the potential drops by at least $\ceil{\log_2 n}-1$. In the first case the potential drop comes from the fact that $d_{u'} = d_u - 1$ and $l_{u'} < l_u$, while in the second case we have $d_{u''} \leq d_{u'} + 1 = d_u$ and $l_{u''} \leq l_{u} - \ceil{\log_2 n}$.

This completes the proof for the claim that with probability at least $\frac{1}{4e}$ every $8 \ceil{\log_2 n}$ rounds the potential of $v$ decreases by at least $\ceil{\log_2 n}-1 > \ceil{\log_2 n}/2$ until it is zero and there is a sequence of successful and collision-free transmission from $s$ to $v$. The expected time for such a sequence to appear is thus a constant times the initial potential of $v$, which is at most $D + 2\ceil{\log_2 n}^2$.
This is because the level of $v$ in $G$ is at most $D$, and the distance label $d_u$ is at most $2 \ceil{\log_2 n}$.
A Chernoff bound furthermore shows that the probability of not finding such a sequence is exponentially concentrated around this mean.
In particular, after $C (D + 2\ceil{\log_2 n} + k \ceil{\log_2 n})$ rounds we expect at least $C'(2D/\ceil{\log_2 n} + 4\ceil{\log_2 n} + k)$ sets of $8 \ceil{\log_2 n}$ rounds in which the potential of $v$ drops at least by $\ceil{\log_2 n}/2$ for any constant $C'$ and $C$ sufficiently larger than $C'$. Furthermore, the probability that there are less than $(2D/\ceil{\log_2 n} + 4\ceil{\log_2 n}$ such round is exponentially small in the expectation, that is, at most $2^{-(2\ceil{\log_2 n} + k)}$.

\end{proof}

We remark that one can get a routing-based $O(D + k \log^2 n)$ broadcast algorithm based on the MGBFS schedule using a similar backward analysis as conducted for network coding. More interestingly one can also use the MGBFS schedule to deliver at least half of the messages to all nodes in time $\tilde{O}(D + k \log n + \log^2 n)$. This can be used together with any forward error correcting (FEC) code to give an algorithm with (essentially) the same complexity as our network coding algorithm. This is interesting because this FEC scheme allows nodes to keep less messages around for coding, and because there are FEC codes with nice extra properties like linear decoding and encoding complexity. Another way to significantly reduce the coding and memory complexity of intermediate nodes is to use the finite-memory variants of random linear network coding introduced in \cite{6089559,6033713}. We defer the details for these algorithms to the journal version of this paper, but mention here that these applications nicely demonstrate that the MGBFS schedule is indeed the right generalization of \cite{GPX05} for multiple messages.


\iffalse
Bernhard says:

Here are some details for proving the message pipelining for routing:

We assume an ordering of the messages. Each message keeps a distinct window of length $\Theta(log^2 n)$ in which to send a message. The window starts at time $d_u + l_u \log n $. If the schedule tells it to send a message and it has the message whose window is active it sends it and otherwise it remains silent or sends noise. We say that a message $\pi$ is late by $x$ rounds at a node $u$ if $u$ learn about $\pi$ for the first time at round $d_u + l_u \log n + x$. We should be able to show that fast links do not add any extra lateness while slow links add in expectation $\log n$ rounds of extra lateness in expectation (and with exponential tail).
Summing up these latenesses over all $\log n$ slow links will lead to a $\Theta(\log^2 n)$ expected delay and this delay is also met with high probability. This completes the proof (sketch) that whp ever node receives every message at time no later than $D + log n \cdot \log n + k \log^2 n$.

Cutting the window size to $\Theta(log n \log \log n)$ gives a probability of at most $\log^{-\Theta(1)} n$ for each message to die out. The proof is almost the same.

\fi

\iffalse
{\bfseries Remarks} (about some subtleties):
\begin{itemize}	
	\item The relaying of fast transmission is important (for network coding) since otherwise there is a $50\%$ chance that a degree of freedom falls of a wave because of an unsuccesful transmission. This probability can be decreased to a negligilbe $1/n$ by increasing the field size $q$ but this also increases the number of coefficient vectors to union bound.
	\item While fast transmissions can in principle pick up new messages from the middle of a stretch this is not possible with relaying anymore. It is thus important that the directed edge in $G'$ only go out of the beginning of a fast stretch. This still suffices to make the diameter of $G'$ logarithmic even so not any shortest-path in $G$ can be used to show this.
	\item The fact that fast steps are spaced out and pipelined according to levels in $G$ while slow steps are spaced out according to levels in $G'$ makes it necessary to schedule fast and slow transmission in separate rounds. This leads to a constant factor of $2$ in front of the diameter term $D$ of the complexity. By scheduling more fast then slow exchanges this constant factor can be reduced to $1+\eps$.
	\item \bcomment{It might still be possible to show that the MGBFS schedule together with any simple oblivious queuing strategy works by reducing the analysis to the throughput of a line network of length $log n$:}\\
	
Any oblivious queuing strategy that delivers $k$ out of $k$ messages over $n'$ queues with probability at least $1-\eps$ in $T(k,n',1-\eps)$ rounds gives a $2R + T(k,\log n,1-\eps)$ multicast algorithm.\\

Any oblivious queuing strategy that delivers $k$ out of many messages over $n'$ queues with probability at least $1-\eps$ in $T(s,k,n',1-\eps)$ rounds can be used, together with a forward forward error correction code, to give a $2R + T(k,\log n,1-\eps)$ multicast algorithm.

\item Simple FEC examples: forwarding a random packet fails badly; forwarding the latest received packet gives delivers $O(k/\sqrt{\log n})$ packets after having put in $O(k + \log 1/\eps)$ with probability $1-\eps$ and thus leads to a $O(D + k\log^{1.5} + \log^2 n)$ algorithm. This beats the routing lower bound but is non-optimal. The optimal oblivious queuing strategy should be for each node to send the message that has been sent least often. We suspect that this might lead to an optimal algorithm.

\item Advantages of using an FEC algorithm over the network coding: With network coding relay nodes need to invest significant time (or storage) for rank computations and generating new vectors. The sinks furthermore have to invest $O(k^3)$ time in solving the dense system of linear equations for decoding. When using error correction codes only the sender needs to create coded packets and only the receivers need to decode. There are furthermore very efficient forward error correction codes known for which this can be done in linear time. Lastly, network coding requires to include the coefficients in the header. This overhead is linear in the number of packets coded together. FEC codes have a much lower overhead.

\item When using the strategy that only the latest message is kept one has furthermore the advantage that each relay node only needs to store one packet. Recent work on finite buffer network coding \cite{} shows that the same can be done for network coding. The same analysis as above can be used to show that if every relay node only keeps one packet and when receiving a new packet updates this packet to a random linear combination of the new and the stored packet the same performance as proven above is obtained.

\item Network coding is the optimal strategy in the following sense: Given any fixed strategy to create a schedule (finite buffer) network coding is optimal, i.e., if a schedule does not allow for a network coding solution then there exists none. Similarly there exists a solution using reduced buffers at the relays only if there exists a linear network coding solution \cite{}.

\end{itemize}
\fi
} 

==> UB_NC.tex <==
\section{Multi-Message Broadcast in Known Topology Setting}\label{sec:multiBC}
In this section, we present a multi-message broadcast algorithm for known topology networks which runs with high probability, in $O(D +k \log n + \log^2 n)$. In the next section, we explain how this algorithm can be extended to the radio network with unknown topology which have collision detection. To the best of our knowledge, the $O(D +k \log n + \log^2 n)$ algorithm we present in this section is the first algorithm that achieves achieves this asymptotically optimal running time (even) in the known topology scenario. 

This section is organized as follows. In \Cref{sec:schedule} we modify the gathering BFS-tree schedule from \cite{GPX05} to allow the streamlined broadcast of not just one but multiple messages. In \Cref{sec:NCalgorithm}, we combine this schedule with the standard distributed implementation of random linear network coding (RLNC). While the algorithm is relatively easy to describe its analysis requires the use of recent advances in analyzing network coding performance from \cite{Haeupler11} in a novel way, which we call \emph{backwards projection analysis}. We describe network coding in \Cref{sec:NCintro} and explain the backwards projection analysis on a simpler example in \Cref{sec:NCanalysis} before we give the complete analysis of our network coding algorithm in \Cref{sec:NCalgorithm}. % and discuss the possibility of replacing the network codes in our fast implementation by forward error correction codes, a simpler form of coding.

%We also show that using only forward error correction codes at the source and sinks it is possible to almost match the performance of network coding with a $O(D +k \log n + \log^2 n) \log \log n$ and give a candidate that might remove the additional $\log \log n$ factor.


\subsection{The Modified Gathering BFS-tree Schedule}\label{sec:schedule}

Our framework is essentially taking the transmission schedule of \cite{GPX05} used on top of GST and extending it to multiple messages. This idea was also attempted in \cite{GP} but its correctness was disproved \cite{QinPersonalCommunication}.

Unfortunately while the schedule in \cite{GPX05, GP} works well in transmitting one message, it cannot be used to pipeline multiple messages directly. The reason is that the analysis of \cite{GPX05} which proves progress of propagation along the tree relies crucially on the fact that nodes that are supposed to send but do not know the message remain silent. This is not possible when multiple messages are to be transmitted since these nodes are making progress on other messages. Instead we modify the schedule of \cite{GPX05} to continue making progress on one message even if other senders (which do not know the message) send noise instead of being silent. In the following, we explain our transmission schedule for broadcasting multiple messages atop GST.

%We use a gathering rank-labeled BFS-tree as introduced in \cite{GPX05}. A rank-labeled BFS-tree is a BFS-tree rooted at the source $s$. We assume the standard notions of levels and parent-child-descendant relationships. We assign each node a rank by the following inductive labeling rule: Each leave has rank $1$; a node with $l$ children of rank $r_1 \geq r_2 \geq \ldots \geq r_l$ has a rank $r_1$ if $r_1 > r_2$ and $r_1+1$ otherwise. A rank-labeled BFS-tree is called gathering if any node of rank $i$ on level $l$ is adjacent to at most one node of rank $i$ at level $l-1$. The existence of such a gathering rank-labeled BFS-tree was proven in \cite{GPX05}:
%
%\begin{lemma}[\cite{GPX05}]\label{lem:gathering}
%For any graph and any node $s$ a gathering rank-labeled BFS-tree rooted at $s$ can be found in polynomial time. Furthermore, the maximum rank of any rank-labeled BFS-tree is at most $\ceil{\log_2 n}$.
%\end{lemma}

The labeling of the gathering BFS-tree defines stretches along which messages can get pipelined fast. In particular, it is possible to pipeline messages along tree-paths that have the same rank without conflicts. We add special directed edges indicating these fast transmission paths. More formally, for a graph $G$ and a gathering spanning tree $T$, we create an imaginary graph $G'$ as follows: we add a directed fast edge from every node $u$ with rank $r$ at level $l$ to every descendant of $u$ in $T$ with rank $r$. We note that, while the diameter of $G$ is $D$, the shortest (directed) path from $s$ to every node $u$ in $G'$ is at most $2\ceil{\log_2 n}$ long. To see this, consider the path from $u$ to $s$ in $T$. On this path, the rank never decreases, thus increases at most $\ceil{\log_2 n}$ times. Furthermore, every stretch on which the rank stays the same corresponds to a directed link in $G'$. Using this, we get the path of length at most $2\ceil{\log_2 n}$ from $s$ to $u$ in $G'$. We use the notation $d_u$ to denote the length of the shortest (directed) path from $s$ to $u$ in $G'$. Thus, $d_u \leq 2\ceil{\log_2 n}$. Equipped with these three labels -- $l_u$ (the BFS layers), $r_u$ (the ranks in the GST) and $d_u$ (the directed distance from the source $s$ in $G'$), we can now define the following schedule \emph{modified gathering BFS-tree (MGBFS) schedule}:

%create a collision free schedule using a modification of the method in \cite{GPX05}.

\begin{definition}[MGBFS schedule]\label{def:schedule}
Given a graph $G$ with a rank-labeled gathering BFS-tree $T$ and a distance label $d$ of $G'$, the MGBFS schedule is defined as follows:
%At the beginning of each round $t$ and each level $l$ we draw a uniformly random integer $i_{t,l}$ from $\{1,2,\ldots,\ceil{\log_2 n}\}$.
The schedule alternates between fast and slow transmissions with fast transmissions only happening when $t \equiv 0 \pmod{2}$ and slow transmissions only happening when $t \equiv 1 \pmod{2}$.
A node $u$ at level $l$ with rank $r$ and distance label $d$ performs a fast transmission if $t \equiv 2(l + 3r) \pmod{6\ceil{\log_2 n}}$, and a slow transmission with probability $2^{-((t-1-2d)/6 \mod \ceil{\log_2 n})}$
if $t \equiv 1 + 2d \pmod{6})$.
\end{definition}

We note that the MGBFS schedule uses fast exchanges exactly as before to pipeline messages towards nodes far away from the source in $G$. The main and crucial modification of the schedule compared to \cite{GPX05,GP} lies in defining the levels of slow exchanges with regards to $G'$ and not $G$. This results in slow exchanges not trying to push messages away from the source themselves but instead they tend to push messages towards entry points of fast stretches (even if this results in going backwards). While this modification on the schedule is only minor a new potential based backwards analysis is needed to prove that this schedule remains efficient even if uninformed nodes broadcast noise.

To prove the new schedule efficient we first show that it is collision free:

\begin{lemma}
In MGBFS schedule, there are no collisions between any two fast transmissions or between any fast and any slow transmission.
\end{lemma}

\begin{proof}
Since fast and slow transmission only happen during even and odd rounds, respectively, it is clear that collisions can only happen between two slow or two fast transmissions.
To see that two fast transmission do not collide, we note that only levels $l$ with $l \equiv t/2 \pmod{3}$ have transmissions since for a fast transmission to happen we need at least $t \equiv 2l + 6r \equiv 2l \pmod{6}$. Since nodes whose levels differ by at least $3$ can not share a neighbor this guarantees that collisions are only caused by nodes within the same level. Two nodes within the same level are furthermore only performing a fast transmission if their ranks $r$ and $r'$ are equivalent modulo $\ceil{\log_2 n}$. By definition of GST, this implies that their ranks are equal and the \emph{collision-freeness} property of GST then guarantees that two such nodes do not share a neighbor in the next level. This shows that there are indeed no collisions between any two fast transmission.
\end{proof}


In the absence of collisions for fast transmission one can see from \Cref{def:schedule} that fast transmissions pipeline nicely. We will use this pipelining to quickly transmit messages from the node at the beginning, that is with smallest level $l$, of a fast-stretch to all nodes on the stretch. For this we make the following rule. Whenever a node in the middle of a fast stretch has to send a message it chooses to relay the last message it has received during a fast transmission from its parent in $T$. This way we get the following property:

\begin{lemma}\label{lem:progslow}
In MGBFS schedule, if node $u$ with level $l$ is the beginning of a fast stretch in $T$ sends a message at time $t$ during a fast transmission then any node $v$ with level $l'>l$ on the same fast stretch will receive this message not later than at time $t' = t + 2(l'-l)$.
\end{lemma}

\noindent
For slow transmissions we get the following progress guarantee:

\begin{lemma}\label{lem:progfast}
For any node $u$ with distance label $d$ if there is at least one node $v$ connected to $u$ in $G$ with distance label $d-1$ then with probability at least $\frac{1}{2e}$ node $u$ receives a message from one such node within any fixed span of $6\ceil{\log_2 n}$ rounds.
\end{lemma}

\begin{proof}
Let $x$ be the number of neighbors of $u$ with distance label $d-1$. Note that within any span of $6 \ceil{\log_2 n}$ rounds there is a round in which all nodes in level $d-1$ send a message independently with probability $p$ between $\frac{1}{x}$ and $\frac{1}{2x}$ while all nodes with distance label $d$ and $d+1$ and thus also all other neighbors of $u$ are silent. The probability that $u$ receives a message from any particular neighbor in this round is at least $\frac{1}{2x} (1 - \frac{1}{x})^{x-1} > \frac{1}{2ex}$. These events are mutually exclusive and we thus get that the total probability for at least one neighbor successfully transmitting to $u$ during this round is at least $\frac{1}{2e}$.
\end{proof}



\subsection{An Optimal Network Coded Broadcast}

In this section, we show how network coding can be used to broadcast $k$ messages in
$O((D + k \log n + \log n)\log n)$ rounds, with high probability.
We then improve this to $O(D + k \log n + \log^2 n)$ using a combination of network coding and the MGBFS schedule defined earlier.
Before getting involved to the details of the algorithms and the analysis, we first give a brief description and introduction to network coding, in particular the standard distributed implementation of Random Linear Network Coding (RLNC).

\subsubsection{Random Linear Network Coding}\label{sec:NCintro}

Using network coding, nodes can mix messages before forwarding. This is in contrast with the traditional ``store and forward'' paradigm in which messages are simply forwarded without being combined. One of the benefits of using network coding is in increasing capacity in networks.

Network Coding was introduced by Ahlswede et at. \cite{ACLY} and extended to RLNC by \cite{HKMKE}. There also a distributed implementation for network coding was suggested. The first use of network coding in gossip-type information dissemination was in \cite{deb2006algebraic}. Lastly, the projection analysis used here can be found in \cite{Haeupler11}.

%\iffalse
%When routing, a node that has multiple messages and is sending has to decide which message to send. This can become a bottleneck, since in a broadcast setting each of its receivers might need a different message.
%%The idea of RLNC network is to send a (random linear) mixture of all messages a node has.
%For example, consider the setting setting where a node $v$ is connected to $k$ other nodes and knows all $k$ messages, while each of its neighbors knows a different subset of $k-1$ out of the $k$ messages. When routing messages, it takes at least $k$ transmissions of $v$ to inform all its neighbors about the missing message. A more efficient solution is to send the XOR of all $k$ messages. Upon receiving this in the first round, each neighbor can XOR the $k-1$ messages it has, and thus obtain the one missing message it needs.
%Linear network coding generalizes this idea to networks.
%\fi

In random linear network coding, a message is regarded as a vector $\vec{m}$ over a finite field $\Fq^l$, where $q$ is an arbitrary prime or prime power.
In the setting of multiple messages $\vec {m_1},\ldots,\vec {m_k}$ network coded packets consist of a linear combination of messages $\vec m = \sum_{i=1}^k \mu_i \vec {m_i} \in \Fq^l$ and a vector of coefficients $\vec \mu = (\mu_1,\ldots,\mu_k) \in \Fq^k$. Because of linearity, a node that knows some of these packets can create a packet of this form for any coefficient combination that is spanned by the coefficient vectors of the packets (and messages) known to it. Also, given a set of $k$ packets with linearly independent coefficient vectors one can reconstruct all messages using Gaussian elimination. Now, the algorithm can be simply described:

Every node $u$ stores all received packets, and maintains the subspace that is spanned by them. Whenever a node decides to transmit, it chooses a random coefficient vector from the subspace by taking a random linear combination of the coefficient vectors stored, and creates a new packet to transmit. Every time a node receives a new packet, it updates its subspace, and if the subspace spanned by the coefficient vectors is the full space, it reconstructs all messages.

%\iffalse
%\bcomment{This is a paste and copy from an earlier NC paper so some reformulation is needed}
%
%The RLNC algorithm sends out packets in the form of vectors over a finite field $\Fq$, where $q$ is an arbitrary prime or prime power. We assume that there are $k$ messages, $\vec {m_1},\ldots,\vec {m_k}$, that are vectors from $\Fq^l$ of length $l$. Every packet that is sent around during the execution of the algorithm has the form $(\vec \mu,\vec m)$, where $\vec m = \sum_{i=1}^k \mu_i \vec {m_i} \in \Fq^l$ is a linear combination of the messages, and $\vec \mu = (\mu_1,\ldots,\mu_k) \in \Fq^k$ is the vector of the coefficients. If enough packets of this form are known to a node, i.e., the span of the coefficient vectors is the full space $\Fq^k$, Gaussian elimination can be used to reconstruct all messages. For this, only $k$ packets with linearly independent coefficient vectors are needed. Linearity furthermore guarantees that any new packet that is created by taking a linear combination of old packets has the same valid format. With this, it is easy to see that a node can produce any packet whose coefficient vector is spanned by the coefficient vectors of the packets it knows. The algorithm is now easily described:
%
%Each node $v$ maintains a subspace $X_v$ that is the span of all packets known to it at the beginning and received so far by simply storing all received packets. If $v$ does not know any messages at the beginning, then $X_v$ is initialized to contain only the zero vector. If $v$ knows some message(s) $\vec m_i$ at the beginning, $X_v$ is initialized to contain the packet $(\vec \mu,\vec {m_i})$ in which $\vec \mu$ is the $i^{\text{th}}$ standard basis vector. $X_v$ also contains all linear combinations that complete the span of these packet(s).
%Whenever node $v$ sends out a packet, it chooses a uniformly random packet from $X_v$ by taking a random linear combination of the stored packets. At the end of each round, all received packets are added to $X_v$ and again the span is taken. If the subspace spanned by the coefficient vectors is the full space, a node decodes all messages.
%
%\bcomment{End of copy}
%\fi


\subsubsection{Analyzing Network Coding}\label{sec:NCanalysis}

In this section, we show that, network coding can be used with a simple BFS-tree schedule to disseminate $k$ messages in $O((D + k + \log n) \log n)$ rounds. This is interesting in its own right and also serves as a simple way to explain our new backwards projection analysis in isolation. This is a helpful preparation for the next part where we will use this analysis together with the more complicated MGBFS-schedule to obtain the optimal $O(D)$ dependence. 

Here, we assume the single-source broadcast setting in which all $k$ messages are initially at the source node $s$.
We furthermore assume that each node $u$ knows its distance $l_u$ to $s$. Having this, nodes communicate in phases.
A phase starts with all nodes at level $l \equiv 0 \pmod{3}$ performing a $\log n$ round iteration of the Decay algorithm,
that is, broadcasting with probability $2^{-i}$ with $i$ varying from $1$ to $\ceil{\log_2 n}$.
To complete a phase, the same process is repeated for all nodes $u$ with distance $l_u \equiv 1 \pmod{3}$, and then for all nodes $u$ with distance $l_u \equiv 2 \pmod{3}$. Whenever a node decides to send, it uses the network coding protocol described in \Cref{sec:NCintro} to construct the packet.

\begin{lemma}\label{lem:simpleNC}
Broadcasting $k$ messages from $s$ to all nodes takes, with high probability, $O((D + k + \log n) \log n)$ rounds, where $D$ diameter of the network.
\end{lemma}

We will use the projection technique from \cite{Haeupler11} to analyze the propagation of knowledge during the random linear coding procedure. In essence this technique only requires to show that one message floods the network sufficiently fast if every node knowing it sends out packets that are informative about the message, with constant probability. An exponential tail bound on this flooding process then directly gives results for $k$ messages. Note that this is exactly the flooding process analyzed \cite[Claim 3.2.]{GPX05} and many other places \underline{except} that we now have to assume that nodes that are scheduled to send but do not know the message are sending noise are thus still causing collisions. This makes a big difference and kills the original analysis. While it is a priori not clear that information still spreads quickly we recover something closely resembling the original proof using our new backwards analysis. 
 
{
For the projection analysis part of the proof we need the following crucial definition and easy to verify facts:

\begin{definition}[{\cite[Definition 4.1.]{Haeupler11}}]
A node knows a coefficient vector $\mu \in GF(2)^k$ if it has received a packet with a coefficient vector $c \in GF(2)^k$ that is not orthogonal, that is, $\left\langle \mu,c \right\rangle \neq 0$.
\end{definition}


\begin{proposition}[{\cite[Lemma 4.2.]{Haeupler11}}]\label{prop:NCfacts}
If a node knows a coefficient vector and sends a packet to a node $v$ then this node $v$ afterwards knows $\mu$ with probability at least $1/2$. Furthermore, if a node knows all $2^k$ coefficient vectors it can decode.
\end{proposition}

\begin{proof}[Proof of \Cref{lem:simpleNC}]
We claim that for any non-zero vector $\mu$ the probability that any fixed node $v$ does not learn $\mu$ within $O((D + k + \log n)\log n)$ rounds is at most $2^{-(k + 2 \log n)}$. From this we conclude via a union bound over all $2^k$ coefficient vectors and all nodes that with high probability all nodes know all coefficient vectors. It then follows from \Cref{prop:NCfacts} that all nodes can decode.

For a node $v$ to learn a fixed coefficient vector $\mu$ there has to exist a sequence of collision-free transmissions from $s$ to $v$. Furthermore, these transmission must carry a coefficient vector that is non-orthogonal to $\mu$. According to \Cref{prop:NCfacts} for any given collision-free transmission there is an independent $1/2$ probability for this to happen. These probabilities are not just independent between each other but are also independent from which nodes send and receive (collision-free) transmissions. We can thus assume that first all collision-free transmissions are determined and then independently each such transmission fails (with respect to $\mu$) with probability $1/2$. Given this we show next that one can find a succesful sequence of transmissions from $s$ to $v$ with probability at least $1 - 2^{-(k + 2 \log n)}$. We will analyze the progress of finding such a sequence by going backwards in time. While this seems not to make a big difference it is crucial and makes the proof that would otherwise seem doomed almost magically easy.

More precisely, our backwards analysis looks at times between $T$ and $1$ and defines a node $v$ at level $l$ to have $d$ successes at time $t$ if there is a node $u$ at level $l-d$ such that there is a sequence of successful and collision-free transmission from $u$ to $v$ between time $t$ and $T$. Thus at most $D$ successes are needed for a node $v$ to learn $\mu$. Furthermore, we will show that in each phase any node $v$ has a constant probability to land at least one success. For this let $v$ have $d$ successes so far and let $u$ be a node with on level $l-d$ having the sequence of successful and collision-free transmission to $v$. Between $t - 3\ceil{\log_2 n}$ and $t$ there is a full iteration of the Decay protocol performed by the nodes in level $l-d-1$ and according to \Cref{lem:progfast} there is thus a constant probability that $u$ receives a collision-free transmission from one of these nodes. With constant probability this transmission is furthermore successful with respect to $\mu$. Therefore there is always an independent constant probability for each phase to generate a success. After $\Theta(D + k + \log n)$ phases the expected number of successes is thus $\Theta(D + k + \log n)$ and due to standard Chernoff bounds the chance that there are less than $D$ successes is at most $2^{-\Theta(D + k + \log n)}$.
\end{proof}

}

\subsubsection{Our Network Coded Broadcast}\label{sec:NCalgorithm}

In this section, we show that using the network coding protocol of \Cref{sec:NCintro} to create packets for the MGBFS schedule results in a fast broadcast algorithm.

The algorithm description is simple.
We use the MGBFS to decide which node sends at what round.
Each time a node decides to sent, it creates a packet using network coding by combining the messages it has received earlier.
Note that we still stick with the rule that intermediate nodes in a fast stretch do {\em not} create packets for a fast transmission, but simply relay the message they received during the fast transmission round.

\begin{lemma}
Suppose we use the MGBFS schedule with random linear network coding to transmit $k$ messages from the source $s$ to all nodes. Then, with high probability, after $O(D + k\log n + \log^2 n)$ rounds all nodes can decode all messages.
\end{lemma}

{
\begin{proof}
As in the proof of \Cref{lem:simpleNC}, we will use the projection technique of \cite{Haeupler11} and analyze the spreading of one coefficient vectors $\mu$ to one node $v$. We do this again by going backwards in time and finding a path of collision-free transmission from $v$ to the source $s$ that is successful \emph{with respect to} $\mu$.
We show that $T = O(D + k\log n + \log^2 n)$ rounds suffice to find such a path with probability at least $1 - 2^{-(2\log n + k)}$.
As before, a union bound over all nodes and all vectors then finishes the proof, and shows (together with \Cref{prop:NCfacts}) that every node can decode.

For any $t$, going backwards in time from time $T$, we will track the set $U_t$ of nodes that are connected to $v$ by a sequence of successful and collision-free transmissions. We then define the potential of $v$ at time $t$ to be $\min_{u \in U_t} d_u \ceil{\log_2 n} + l_u$. We will show that this potential decreases with probability at least $\frac{1}{4e}$ by at least $\ceil{\log_2 n}-1$ every $8\ceil{\log_2 n}$ rounds.

We start with the case where the node $u \in U_t$ that minimizes the potential of $v$ has at least one neighbor at level below it in $G'$. In this case, \Cref{lem:progslow} guarantees that with probability at least $\frac{1}{2e}$ during the rounds between $t - 6 \ceil{\log_2 n}$ and $t$ there is a collision-free transmission from a node $u'$ with $d_{u'} = d_u - 1$ to $u$, and is successful with respect to $\mu$, with probability $1/2$.
Since $u'$ and $u$ are neighbors their levels $l_u$ and $l_{u'}$ differ at most by one, thus a successful transmission decreases the potential by at least $(d_u \ceil{\log_2 n} + l_u) - (d_{u'} \ceil{\log_2 n} + l_{u'}) = (d_u - d_{u'})\ceil{\log_2 n} - (l_u - l_{u'}) \geq \ceil{\log_2 n} - 1$. Thus, if $u$ has a neighbor with a distance label lower than $d_u$
then with probability at least $\frac{1}{4e}$ the potential decreases by at least $\ceil{\log_2 n} - 1$ within any $8 \ceil{\log_2 n}$ rounds.

In the second case, the node $u \in U_t$ that minimizes the potential of $v$ at time $t$ does not have a neighbor with a lower distance label.
For this case, we need to understand the behavior of fast stretches. We first observe that the start node of any fast stretch initiates a ``transmission wave'' every $6 \ceil{\log_2 n}$ rounds by creating a new message and sending it as a fast transmission. This message gets then pipelined through the fast stretch with one progress every fast transmission rounds (that is every two rounds) until the message reaches the end of the stretch. For any node on a fast stretch there is thus a new wave arriving every $6\ceil{\log_2 n}$ rounds and each of these waves is successful with respect to $\mu$ with probability at least $1/2$.

Note that the second case can only happen if $u=s$ or if there is one directed edge in $G'$ representing a fast stretch going into $u$ originating from a node $u'$ one level below $u$ in $G'$.
Thus, at a time $t'$ between $t-6 \ceil{\log_2 n}$ and $t$, a fast transmission wave arrives in $u$ and with probability $1/2$ leads to an extended sequence of collision-free transmissions that are successful $\mu$.
In particular, if the wave originated from $u'$ during the rounds $t'-2 \ceil{\log_2 n}$ and $t'$ then there is a sequence of transmission from $u'$ to $v$ between time $t - 8 \ceil{\log_2 n}$ and $T$, and otherwise the wave propagated for $\ceil{\log_2 n}$ steps and there is a node $u''$ between $u'$ and $u$ on the fast stretch with a sequence of transmission to $v$ starting at time $t - 8 \ceil{\log_2 n}$. In both cases the potential drops by at least $\ceil{\log_2 n}-1$. In the first case the potential drop comes from the fact that $d_{u'} = d_u - 1$ and $l_{u'} < l_u$, while in the second case we have $d_{u''} \leq d_{u'} + 1 = d_u$ and $l_{u''} \leq l_{u} - \ceil{\log_2 n}$.

This completes the proof for the claim that with probability at least $\frac{1}{4e}$ every $8 \ceil{\log_2 n}$ rounds the potential of $v$ decreases by at least $\ceil{\log_2 n}-1 > \ceil{\log_2 n}/2$ until it is zero and there is a sequence of successful and collision-free transmission from $s$ to $v$. The expected time for such a sequence to appear is thus a constant times the initial potential of $v$, which is at most $D + 2\ceil{\log_2 n}^2$.
This is because the level of $v$ in $G$ is at most $D$, and the distance label $d_u$ is at most $2 \ceil{\log_2 n}$.
A Chernoff bound furthermore shows that the probability of not finding such a sequence is exponentially concentrated around this mean.
In particular, after $C (D + 2\ceil{\log_2 n} + k \ceil{\log_2 n})$ rounds we expect at least $C'(2D/\ceil{\log_2 n} + 4\ceil{\log_2 n} + k)$ sets of $8 \ceil{\log_2 n}$ rounds in which the potential of $v$ drops at least by $\ceil{\log_2 n}/2$ for any constant $C'$ and $C$ sufficiently larger than $C'$. Furthermore, the probability that there are less than $(2D/\ceil{\log_2 n} + 4\ceil{\log_2 n}$ such round is exponentially small in the expectation, that is, at most $2^{-(2\ceil{\log_2 n} + k)}$.

\end{proof}

We remark that one can get a routing-based $O(D + k \log^2 n)$ broadcast algorithm based on the MGBFS schedule using a similar backward analysis as conducted for network coding. More interestingly one can also use the MGBFS schedule to deliver at least half of the messages to all nodes in time $\tilde{O}(D + k \log n + \log^2 n)$. This can be used together with any forward error correcting (FEC) code to give an algorithm with (essentially) the same complexity as our network coding algorithm. This is interesting because this FEC scheme allows nodes to keep less messages around for coding, and because there are FEC codes with nice extra properties like linear decoding and encoding complexity. Another way to significantly reduce the coding and memory complexity of intermediate nodes is to use the finite-memory variants of random linear network coding introduced in \cite{6089559,6033713}. We defer the details for these algorithms to the journal version of this paper, but mention here that these applications nicely demonstrate that the MGBFS schedule is indeed the right generalization of \cite{GPX05} for multiple messages.


\iffalse
Bernhard says:

Here are some details for proving the message pipelining for routing:

We assume an ordering of the messages. Each message keeps a distinct window of length $\Theta(log^2 n)$ in which to send a message. The window starts at time $d_u + l_u \log n $. If the schedule tells it to send a message and it has the message whose window is active it sends it and otherwise it remains silent or sends noise. We say that a message $\pi$ is late by $x$ rounds at a node $u$ if $u$ learn about $\pi$ for the first time at round $d_u + l_u \log n + x$. We should be able to show that fast links do not add any extra lateness while slow links add in expectation $\log n$ rounds of extra lateness in expectation (and with exponential tail).
Summing up these latenesses over all $\log n$ slow links will lead to a $\Theta(\log^2 n)$ expected delay and this delay is also met with high probability. This completes the proof (sketch) that whp ever node receives every message at time no later than $D + log n \cdot \log n + k \log^2 n$.

Cutting the window size to $\Theta(log n \log \log n)$ gives a probability of at most $\log^{-\Theta(1)} n$ for each message to die out. The proof is almost the same.

\fi

\iffalse
{\bfseries Remarks} (about some subtleties):
\begin{itemize}	
	\item The relaying of fast transmission is important (for network coding) since otherwise there is a $50\%$ chance that a degree of freedom falls of a wave because of an unsuccesful transmission. This probability can be decreased to a negligilbe $1/n$ by increasing the field size $q$ but this also increases the number of coefficient vectors to union bound.
	\item While fast transmissions can in principle pick up new messages from the middle of a stretch this is not possible with relaying anymore. It is thus important that the directed edge in $G'$ only go out of the beginning of a fast stretch. This still suffices to make the diameter of $G'$ logarithmic even so not any shortest-path in $G$ can be used to show this.
	\item The fact that fast steps are spaced out and pipelined according to levels in $G$ while slow steps are spaced out according to levels in $G'$ makes it necessary to schedule fast and slow transmission in separate rounds. This leads to a constant factor of $2$ in front of the diameter term $D$ of the complexity. By scheduling more fast then slow exchanges this constant factor can be reduced to $1+\eps$.
	\item \bcomment{It might still be possible to show that the MGBFS schedule together with any simple oblivious queuing strategy works by reducing the analysis to the throughput of a line network of length $log n$:}\\
	
Any oblivious queuing strategy that delivers $k$ out of $k$ messages over $n'$ queues with probability at least $1-\eps$ in $T(k,n',1-\eps)$ rounds gives a $2R + T(k,\log n,1-\eps)$ multicast algorithm.\\

Any oblivious queuing strategy that delivers $k$ out of many messages over $n'$ queues with probability at least $1-\eps$ in $T(s,k,n',1-\eps)$ rounds can be used, together with a forward forward error correction code, to give a $2R + T(k,\log n,1-\eps)$ multicast algorithm.

\item Simple FEC examples: forwarding a random packet fails badly; forwarding the latest received packet gives delivers $O(k/\sqrt{\log n})$ packets after having put in $O(k + \log 1/\eps)$ with probability $1-\eps$ and thus leads to a $O(D + k\log^{1.5} + \log^2 n)$ algorithm. This beats the routing lower bound but is non-optimal. The optimal oblivious queuing strategy should be for each node to send the message that has been sent least often. We suspect that this might lead to an optimal algorithm.

\item Advantages of using an FEC algorithm over the network coding: With network coding relay nodes need to invest significant time (or storage) for rank computations and generating new vectors. The sinks furthermore have to invest $O(k^3)$ time in solving the dense system of linear equations for decoding. When using error correction codes only the sender needs to create coded packets and only the receivers need to decode. There are furthermore very efficient forward error correction codes known for which this can be done in linear time. Lastly, network coding requires to include the coefficients in the header. This overhead is linear in the number of packets coded together. FEC codes have a much lower overhead.

\item When using the strategy that only the latest message is kept one has furthermore the advantage that each relay node only needs to store one packet. Recent work on finite buffer network coding \cite{} shows that the same can be done for network coding. The same analysis as above can be used to show that if every relay node only keeps one packet and when receiving a new packet updates this packet to a random linear combination of the new and the stored packet the same performance as proven above is obtained.

\item Network coding is the optimal strategy in the following sense: Given any fixed strategy to create a schedule (finite buffer) network coding is optimal, i.e., if a schedule does not allow for a network coding solution then there exists none. Similarly there exists a solution using reduced buffers at the relays only if there exists a linear network coding solution \cite{}.

\end{itemize}
\fi
} 

==> Wrapup.tex <==
\section{Multi-Message Broadcast in Unknown Topology Setting}\label{sec:final}
In \Cref{sec:gather}, we reduce the multiple-source broadcast problem to the single source broadcast problem by describing a simple algorithm that gathers all messages in one node. Then, in \Cref{subsec:wrapup}, we explain the after gathering messages in a center (an elected leader), the distributed broadcast algorithm presented in \Cref{sec:multiBC} can be put together with the Psuedo-GST structures which we constructed in \Cref{sec:GST} to get a distributed $k$-message broadcast algorithm for radio networks with unknown topology and collision detection in $O(D + k\log n + \log^6 n)$ rounds. This time complexity is almost optimal considering the related $\Omega(D + k\log n + \log^2 n)$ lower bound that follows from~\cite{NCLB} and~\cite{ABLP}.

\subsection{Gathering in Known Radio Networks}\label{sec:gather}
%In this section we show how to reduce the multi-source broadcast problem to the single-source broadcast problem. For this, we first describe a simple deterministic centralized gathering algorithm that collects $k$ messages that are distributed over the network arbitrarily, in one node $v$, and in $D + 3k - 4$ rounds. Then we explain how to modify this algorithm to accomplish this gathering goal in a distributed setting with known topology and in $D + O(k \log n)$ rounds.  
%
%\paragraph{The \emph{Centralized Gathering Algorithm} (CGA):} First, constructs a BFS tree rooted at $v$. Then, to avoid collisions within a level, at most one node per level transmits in each round. Furthermore, each node retransmits only the messages of its children and only every third level is allowed to send at any round, hence avoiding collisions between levels. More precisely, in every round $t$, we choose one node at distance $i$ to send (breaking ties arbitrarily), if $i - t = D - 2 \mod 3$.
%
%\begin{lemma}\label{lem:centralized_gathering}
%The CGA Algorithm collects $k$ messages at $v$ within at most $D + 3k - 4$ rounds.
%\end{lemma}
%\fullOnly{
%\begin{proof}
%From the previous discussion, it is clear that no collisions occur during the execution of the algorithm. Since at each level at most one node sends, the graph can be essentially reduced to a line graph of sufficient length in which all messages are at most at distance $D-1$ from the source located at one end of the graph. We note that moving messages away from the source can only increase the number of steps the gathering process takes. For the sake of analysis, we thus move the $i$th message to distance $(D-1) + 3(i-1)$. Running the algorithm on this starting position will move every message exactly one step in each round. The algorithm thus terminates after at most $(D-1) + 3(k-1)$ steps.
%\end{proof}
%
%Note that in a line graph of length $D$ with $v$ on one end and $k$ messages starting at the other end, the gathering process needs at least $D+3k-4$ rounds, thus the above algorithm is optimal even up to the additive constant. BFS-tree based gathering algorithms were used in all previous works on multicast protocols in radio networks. A similar algorithm to the one presented here was given in \cite{FQ06} for gathering messages in the context of gossiping, where each node has exactly one message. In this special case, the gathering can be done slightly faster in $3(n-1)$ rounds.
%%The best distributed algorithm for this problem is \cite{} and runs in ... time. The best deterministic distributed algorithm  is given in \cite{}.
%%\bcomment{discuss that this part is not as easily implementable in a distributed way.}
%}
%
%\medskip
In this section, we show how to reduce the multi-source broadcast problem to the single-source broadcast problem by presenting a distributed algorithm that gathers all $k$ messages in one node. 

\begin{theorem}\label{thm:gather} There exists a distributed algorithm that given a node $v$ gathers all $k$ messages in $v$ in $D + O(k \log n)$ rounds with high probability, where $D$ is the diameter of the network.
\end{theorem}

We call the algorithm for \Cref{thm:gather} the \emph{Gathering Algorithm} (GA). This algorithm assumes that there is a BFS-tree $T$ rooted at a node $v$ such that each node knows its parent in the tree\footnote{It is easy to see that a node knowing its children is also a sufficient condition.}. The algorithm collects all $k$ messages at the root $v$ in $D + O(k \log n)$ rounds with high probability. Using this algorithm with $v$ being the node with the smallest ID and $T$ being the canonical BFS-tree rooted at $v$ leads to \Cref{thm:gather}, since both $v$ and $T$ can be computed locally and consistently with the assumed knowledge of the topology. As a small technical detail, we first present the algorithm for the case where $k$ is polynomial in $n$ and then we explain how to slightly modify this scheme to also cover the less interesting case where $k$ is super-polynomial.

\paragraph{The \emph{Gathering Algorithm} (GA):} For each message residing in a node $u$, this node makes $(c+1)\log n$ copies and draws for each copy a distinct uniformly random delay from $\{1, 2, ..., 10(c+1) k \log n\}$ without replacement. We denote these copies with $\pi_1, \pi_2, \ldots$ and write $t_{\pi}$ for the delay of one such packet $\pi$. The transmissions in GA are now as follows: Initially, each node $u$ transmits each of its own packets $\pi$ in round $3 t_{\pi}$.\footnote{If there are packets $\pi,\pi'$ created at the same node with $t_{\pi} = t_{\pi'}$ we treat this as a collision and send none of these packets. Note that since packet delays for copies of the same message are drawn without replacement this can only happen if the packets $\pi$ and $\pi'$ come from different messages that start at the same node. We furthermore show that it is unlikely that too many of these collisions happen.} In each packet transmitted by a node $u$ the ID of $u$'s parent is attached to indicate for whom this transmission is intended. Other than that, any node $w$ that receives a packet, checks the parent-id field of the packet and if it matches its own ID it retransmits the packet. Retransmissions are done in the immediate next round by simply forwarding the same message but replacing the parent-ID field with the ID of the parent of the retransmitting node. 

In the absence of collisions this leads to each packet getting routed to the root along the tree $T$. Next, we show that the random delays prevent collisions well enough that at least one copy of each message reaches the root with high probability. 

\begin{lemma}\label{lem:distributed_gathering}
For every BFS-tree $T$ rooted at node $v$, the GA algorithm collects all the $k$ messages in node $v$ in $D + O(k \log n)$ rounds with high probability.
\end{lemma}

\begin{proof} First, since the largest random delay is $10(c+1) k \log n$, transmission of each packet is started by round $30(c+1) k \log n$ and because each packet is only retransmitted once in each node on the path down to the root, and these retransmissions are in contiguous rounds, all transmissions are finished by the end of round $Depth(T) + 30(c+1) k\log n \leq D + O(k \log n)$. Now, we show that with high probability, for each message, at least one of its copies gets to the root $v$. 

First, we define the distance of a packet $\pi$ by $dist(\pi) = 3 t_{\pi} + h$ where $h$ is the distance between the root $v$ and the node message $\pi$ resides in initially. Note that this is exactly the number of rounds after which the packet $\pi_i$ reach root node $v$ if no collision occurs. To analyze the likelihood of collisions we define two packets $\pi$ and $\pi'$ to \emph{conflicting} if there exists a time for which transmissions (or retransmissions) of these two packets cause a collision. It is easy to see that because of the method used for retransmissions, $\pi$ and $\pi'$ can only be conflicting if $|dist(\pi_i) - dist(\sigma_j)| \leq 2 $. With this in mind we call a distance value $x$ \emph{occupied} if there is a packet $\pi''$ that has a $|dist(\pi) - x| \leq 2$. Each packet causes at most $5$ distance values to be occupied which leads to at most $5(c+1) k \log n$ distance-values being occupied in total. We will now focus on the $(c+1)\log n$ packets corresponding to one message and show that with high probability at least one of them is not conflicting with any other packet. Since the delay and thus essentially also the distance value of each copy of $m$ is chosen out of $10(c+1) k\log(n)$ different possibilities each packet has a probability of at least $\frac{1}{2}$ to get a distance value that is not occupied by any packet belonging to another message. Note that because the delay values are chosen without replacement these probabilities are not independent but negatively dependent. The probability that none of the chosen delays is to occupied by a packet belonging to another message is thus at most $2^{-(c+1) \log n} = n^{-(c+1)}$. Furthermore since the delays of the copies of a message are distinct their distances differ by at least three and are thus not conflicting. We thus get a probability of $1 - n^{-(c+1)}$ that any particular message has at least one copy that reaches the root and a union bound over all $n^c$ packets shows that with probability at least $1 - 1/n$ all messages have such a copy and are known to the root in the end. 
\end{proof}

\noindent {\bf{Remark}:} {In case $k$ is super-polynomial in $n$, we can simply modify the GA algorithm by blocking messages into block sizes of $\lceil\frac{k}{n^2}\rceil$ message each, treating each message block as a larger message and transmitting each large message using $\lceil\frac{k}{n^2}\rceil$ contiguous rounds. }


\subsection{Putting The Pieces Together} \label{subsec:wrapup}
\dots



